Revisiting Multi-User Downlink in IEEE 802.11ax: A Designers Guide to MU-MIMO

Downlink (DL) Multi-User (MU) Multiple Input Multiple Output (MU-MIMO) is a key technology that allows multiple concurrent data transmissions from an Access Point (AP) to a selected sub-set of clients for higher network efficiency in IEEE 802.11ax. However, DL MU-MIMO feature is typically turned off as the default setting in AP vendors' products, that is, turning on the DL MU-MIMO may not help increase the network efficiency, which is counter-intuitive. In this article, we provide a sufficiently deep understanding of the interplay between the various underlying factors, i.e., CSI overhead and spatial correlation, which result in negative results when turning on the DL MU-MIMO. Furthermore, we provide a fundamental guideline as a function of operational scenarios to address the fundamental question "when the DL MU-MIMO should be turned on/off".

==> tmp.tex <==
\section{Demos}

%figures:
% Double column:
\begin{figure*}[t]
    \centering
    \includegraphics[width = .8\textwidth]{tier.png}
    \caption{Illustration of three-tier structure: AP $1$ selects two 20 MHz sub-channels in 2.4 GHz band, two 20 MHz sub-channels in 5 GHz band, and a 20 MHz channel in 6 GHz based on a certain policy $\pi$. Then AP $1$ allocates these $5$ resource units to its attached stations.}
    \label{fig:tier}
\end{figure*}

%normal:
\begin{figure}[t]
    \centering
    \includegraphics[width=.43\textwidth]{Performance.eps}
    \caption{Average throughput comparison.}
    \label{fig:performance}
\end{figure}

%multi figures
\begin{figure}[htbp] 
  \centering
  \subfigure[Total utility vs the number of URLLC user numbers per Mini-slot. ] {\includegraphics[width=.4\textwidth]{max_rate.eps}}\quad
  \subfigure[ The $\frac{\Phi(n)}{DRC(n)}$ of each eMBB user, $M = 8$ per mini-slot.] {\includegraphics[width=.4\textwidth]{mr_fair.eps}}
  \caption{Simulation result with the objective of maximizing total rate, i.e., $U(\Phi(n)) = \Phi(n)$.}
  \label{fig:mr}
\end{figure}
